Support for Non-conformal Meshes in PETSc's DMPlex Interface

PETSc's DMPlex interface for unstructured meshes has been extended to support non-conformal meshes. The topological construct that DMPlex implements---the CW-complex---is by definition conformal, so representing non- conformal meshes in a way that hides complexity requires careful attention to the interface between DMPlex and numerical methods such as the finite element method. Our approach---which combines a tree structure for subset- superset relationships and a "reference tree" describing the types of non-conformal interfaces---allows finite element code written for conformal meshes to extend automatically: in particular, all "hanging-node" constraint calculations are handled behind the scenes. We give example code demonstrating the use of this extension, and use it to convert forests of quadtrees and forests of octrees from the p4est library to DMPlex meshes.

==> tikzlibrary3d.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary3d.code.tex,v 1.2 2013/07/17 10:36:34 tantau Exp $



% New coordinate systems:

\tikzdeclarecoordinatesystem{xyz cylindrical}
{%
  \pgfset{/tikz/cs/.cd,angle=0,radius=0,z=0,#1}%
  \pgfpointcylindrical{\tikz@cs@angle}{\tikz@cs@xradius}{\tikz@cs@z}%
}

\tikzdeclarecoordinatesystem{xyz spherical}
{%
  \pgfset{/tikz/cs/.cd,angle=0,radius=0,latitude=0,longitude=0,#1}%
  \pgfpointspherical{\tikz@cs@angle}{\tikz@cs@latitude}{\tikz@cs@xradius}%
}

\pgfset{/tikz/cs/longitude/.store in=\tikz@cs@angle}
\pgfset{/tikz/cs/latitude/.store in=\tikz@cs@latitude}


% Options for transforming into a plane:

\tikzoption{plane origin}{\def\tikz@plane@origin{\tikz@scan@one@point\pgfutil@firstofone#1}}
\tikzoption{plane x}{\def\tikz@plane@x{\tikz@scan@one@point\pgfutil@firstofone#1}}
\tikzoption{plane y}{\def\tikz@plane@y{\tikz@scan@one@point\pgfutil@firstofone#1}}

\let\tikz@plane@origin=\pgfpointorigin
\def\tikz@plain@x{\pgfpointxy{1}{0}}
\def\tikz@plain@y{\pgfpointxy{0}{1}}

\tikzoption{canvas is plane}[]{
  \tikz@canvas@is@plane
}
\tikzoption{canvas is xy plane at z}{%
  \tikz@addtransform{\pgftransformshift{\pgfpointxyz{0}{0}{#1}}}%
}
\tikzoption{canvas is yx plane at z}[]{%
  \def\tikz@plane@origin{\pgfpointxyz{0}{0}{#1}}%
  \def\tikz@plane@x{\pgfpointxyz{0}{1}{#1}}%
  \def\tikz@plane@y{\pgfpointxyz{1}{0}{#1}}%
  \tikz@canvas@is@plane
}
\tikzoption{canvas is xz plane at y}[]{%
  \def\tikz@plane@origin{\pgfpointxyz{0}{#1}{0}}%
  \def\tikz@plane@x{\pgfpointxyz{1}{#1}{0}}%
  \def\tikz@plane@y{\pgfpointxyz{0}{#1}{1}}%
  \tikz@canvas@is@plane
}
\tikzoption{canvas is zx plane at y}[]{%
  \def\tikz@plane@origin{\pgfpointxyz{0}{#1}{0}}%
  \def\tikz@plane@x{\pgfpointxyz{0}{#1}{1}}%
  \def\tikz@plane@y{\pgfpointxyz{1}{#1}{0}}%
  \tikz@canvas@is@plane
}
\tikzoption{canvas is yz plane at x}[]{%
  \def\tikz@plane@origin{\pgfpointxyz{#1}{0}{0}}%
  \def\tikz@plane@x{\pgfpointxyz{#1}{1}{0}}%
  \def\tikz@plane@y{\pgfpointxyz{#1}{0}{1}}%
  \tikz@canvas@is@plane
}
\tikzoption{canvas is zy plane at x}[]{%
  \def\tikz@plane@origin{\pgfpointxyz{#1}{0}{0}}%
  \def\tikz@plane@x{\pgfpointxyz{#1}{0}{1}}%
  \def\tikz@plane@y{\pgfpointxyz{#1}{1}{0}}%
  \tikz@canvas@is@plane
}



% Transformation code

\def\tikz@canvas@is@plane{
  \pgf@process{\tikz@plane@x}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{\tikz@plane@y}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@process{\tikz@plane@origin}%
  \edef\pgf@marshal{\noexpand\tikz@addtransform{%
      \noexpand\pgftransformtriangle
      {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}
      {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}
      \noexpand\pgftransformscale{0.035146}%
      \noexpand\pgfsetxvec{\noexpand\pgfpoint{1cm}{0cm}}%
      \noexpand\pgfsetyvec{\noexpand\pgfpoint{0cm}{1cm}}%
      \noexpand\pgfsetzvec{\noexpand\pgfpoint{0cm}{0cm}}%
    }}%
  \pgf@marshal%
}

                                    
\endinput


==> tikzlibraryquadtree.code.tex <==
% This file defines macros for making quadtree diagrams in tikz pictures.
% It depends on the tikz library for trees, so you file must include
%
% \usetikzlibrary{trees}
% \usetikzlibrary{quadtree}

% This puts a quadrant centered at the current location.
\def\quadrant{+(-1cm,-1cm) rectangle +(1cm,1cm) (0,0)}

% Morton order growth function
\tikzstyle{morton order}=[growth function=\quadtree@morton,
                          level distance=\quadtree@sqrt2,
   edge from parent path={(\tikzparentnode.center) (\tikzchildnode.center)}]

% Three options that control the placement of leaves

% Places space between leaves: the space is the same at each level, so this only
% works if the size of the leaves is less than the absolute space
\tikzset{quadtree absolute space/.initial=0.0}
% Places space between leaves proportional to the size of the leaves
\tikzset{quadtree relative space/.initial=0.0}
% Shrinks a leaf towards its center (after applying the above spaces)
\tikzset{quadtree scale/.initial=1.0}

\def\quadtree@morton{%
  \ifnum\tikznumberofcurrentchild=1\relax%
    \c@pgf@counta=-135\relax%
  \else\ifnum\tikznumberofcurrentchild=2\relax%
    \c@pgf@counta=-45\relax%
  \else\ifnum\tikznumberofcurrentchild=3\relax%
    \c@pgf@counta=135\relax%
  \else%
    \c@pgf@counta=45\relax%
  \fi\fi\fi
  \pgftransformscale{.5*(1-2^(\the\tikztreelevel-1)*%
(\pgfkeysvalueof{/tikz/quadtree absolute space})-%
(\pgfkeysvalueof{/tikz/quadtree relative space}))}%
  \pgftransformshift{\pgfpointpolar{\the\c@pgf@counta}%
  {\quadtree@sqrt2 * (2 - (1 -2^(\the\tikztreelevel-1)*%
(\pgfkeysvalueof{/tikz/quadtree absolute space})-%
(\pgfkeysvalueof{/tikz/quadtree relative space})))/%
(1-2^(\the\tikztreelevel-1)*(\pgfkeysvalueof{/tikz/quadtree absolute space})-
(\pgfkeysvalueof{/tikz/quadtree relative space}))}}
  \pgftransformscale{(\pgfkeysvalueof{/tikz/quadtree scale})}
}

\def\quadtree@sqrt2{1.41421356237310 cm}

% Example usage:
%
%  \draw [morton order,quadtree absolute space=0.05] coordinate
%    child {[red]\quadrant}
%    child {[green]\quadrant}
%    child {
%      child {[green]\quadrant}
%      child {
%        child {[green]\quadrant}
%        child {[blue]\quadrant}
%        child {[red]\quadrant}
%        child {[green]\quadrant}}
%      child {
%        child {[green]\quadrant}
%        child {[blue]\quadrant}
%        child {
%          child {[green]\quadrant}
%          child {[blue]\quadrant}
%          child {[red]\quadrant}
%          child {[green]\quadrant}}
%        child {[green]\quadrant}}
%      child {[red]\quadrant}
%      child {[green]\quadrant}}
%    child {[blue]\quadrant};


==> tikzlibrarythplex.code.tex <==
% Default styles for thplex tikz pictures

\usetikzlibrary{matrix,arrows}
\usetikzlibrary{decorations,decorations.pathmorphing}

\pgfarrowsdeclare{left triangle 60}{left triangle 60}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfutil@tempdimb=7.29\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=.5\pgfutil@tempdima\advance\pgfutil@tempdimb by\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{150}{9\pgfutil@tempdima}}}
  \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{-180}{6\pgfutil@tempdima}}}
  \pgfpathclose
  \pgfusepathqfillstroke
}

\pgfarrowsdeclare{left stealth'}{left stealth'}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfutil@tempdimb=6\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=2\pgfutil@tempdima\advance\pgfutil@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{2\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-.5\pgfutil@tempdima}{.5\pgfutil@tempdima}}
  {\pgfqpoint{-3\pgfutil@tempdima}{1.5\pgfutil@tempdima}}
  {\pgfqpoint{-6\pgfutil@tempdima}{3.25\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-4.5\pgfutil@tempdima}{2.125\pgfutil@tempdima}}
  {\pgfqpoint{-3.75\pgfutil@tempdima}{-1.0625\pgfutil@tempdima}}
  {\pgfqpoint{-3.75\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{2\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqfillstroke
}

\pgfdeclaredecoration{simple line}{initial}{
  \state{initial}[width=\pgfdecoratedpathlength-1sp]{\pgfmoveto{\pgfpointorigin}}
  \state{final}{\pgflineto{\pgfpointorigin}}
}
\tikzset{
  shift left/.style={decorate,decoration={simple line,raise=#1}},
  shift right/.style={decorate,decoration={simple line,raise=-1*#1}},
}

% physical space
\tikzset{vertex/.prefix style={circle,inner sep=0cm,minimum width=.1414cm,draw=black,fill=black}}
\tikzset{vertexlabel/.prefix style={text=black}}
\tikzset{facet/.prefix style={draw=black}}
\tikzset{facetlabel/.prefix style={text=black}}
\tikzset{cell/.prefix style={fill=none}}

% Hasse diagram
\tikzset{point/.prefix style={circle,draw=black,fill=none,execute at begin node={\strut},inner sep=0cm}}
\tikzset{arrow/.prefix style={-left triangle 60,shift left=0.0mm}}
\tikzset{uparrow/.prefix style={<->,>=latex'}}
\tikzset{downarrow/.prefix style={<->,>=latex'}}
\tikzset{every matrix/.prefix style={anchor=center,column sep=0.5cm}}
\tikzset{every picture/.prefix style={node distance=1.25cm}}
\tikzset{tree/.prefix style={->,decorate,decoration={snake}}}
% vim: set ft=tex :

